NeuralFastLAS: Fast Logic-Based Learning from Raw Data

Symbolic rule learners generate interpretable solutions, however they require the input to be encoded symbolically. Neuro-symbolic approaches overcome this issue by mapping raw data to latent symbolic concepts using a neural network. Training the neural and symbolic components jointly is difficult, due to slow and unstable learning, hence many existing systems rely on hand-engineered rules to train the network. We introduce NeuralFastLAS, a scalable and fast end-to-end approach that trains a neural network jointly with a symbolic learner. For a given task, NeuralFastLAS computes a relevant set of rules, proved to contain an optimal symbolic solution, trains a neural network using these rules, and finally finds an optimal symbolic solution to the task while taking network predictions into account. A key novelty of our approach is learning a posterior distribution on rules while training the neural network to improve stability during training. We provide theoretical results for a sufficient condition on network training to guarantee correctness of the final solution. Experimental results demonstrate that NeuralFastLAS is able to achieve state-of-the-art accuracy in arithmetic and logical tasks, with a training time that is up to two orders of magnitude faster than other jointly trained neuro-symbolic methods.

==> extra.tex <==
\section{Abduction}

Using the $abduce\_possibilities(T, e)$ 
algorithm from FastNonOPL \cite{fastlas2}, we can define the neural abduction 
algorithm described in \autoref{algo:abduce}. 
The symbol $p_\text{as}$ represents the answer 
set of the bottom program that the possibility $p$ 
corresponds to.



\begin{algorithm}
  \caption{abduce\_neural\_possibilities($T$, $e$)}
  \label{algo:abduce}
  \begin{algorithmic}
    \STATE $C = \bigcup_{A \in \AS(P_\Z)} A$
    \STATE $pp_z = \varnothing$ for $z \in \Z$
    \STATE Create a WCDPI $e' = \langle e_\text{id}, \infty, \langle \epiinc, \epiexc \rangle, e_\text{ctx} \cup P_\Z \rangle$
    \STATE poss $= abduce\_possibilities(T, e')$
    \FOR{$p \in \text{poss}$}
      \STATE $z' = p_\text{as} \cap C$
      \STATE $pp_{z'} = pp_{z'} \cup \{ p \}$
    \ENDFOR
    \RETURN $\{ pp_z : z \in \Z \}$
  \end{algorithmic}
\end{algorithm}


Intuitively, the algorithm computes all possibilities 
of an raw-data example by mapping it into 
a WCDPI and using $abduce\_possibilities(T, e)$ \cite{fastlas2}
to get all possibilities of the WCDPI. The 
algorithm leverages the fact that 
$abduce\_possibilities(T, e)$
begins by computing all of the answer sets 
$AS = \AS(\bottom(B \cup e_\text{ctx} \cup P_\Z))$
and then finding possible fixes for each $A \in AS$,
as described in \cite{fastlas2}.
Assuming that $B \cup e_\text{ctx}$ contains no
choice rules, then each answer set in $AS$
maps uniquely to a possible 
latent label 
that satisfy the constraints in $B$ (if any).
If the task is non-observational, the $abduce\_possibilities(T, e)$
will generate a set of possible fixes for each 
of the answer sets.

Once the possibilities have been generated 
by $abduce\_possibilities$, 
we iterate through the answer sets to 
group them by their network latent choices.
$C$ represents 
the flattened set of all possible 
\texttt{nn(}$i$\texttt{,}$\Z_{i,j}$\texttt{)}
which we use to extract the latent choices $z'$
to deduce which group of possibilities a 
possibility should belong to. If the task 
is an OPL task, then each possibility will 
correspond to a unique neural latent output.

\subsection{Solutions to a Task}

To motivate the algorithm of NeuralFastLAS, we define the concept of an 
optimal and correct solution to a task. 


\begin{definition}[Collapse of a NeuralFastLAS Task]
Let $T = \langle B, M, E^*, \Z \rangle$ be a 
NeuralFastLAS task, we define 
the \textit{collapse of $T$} into a normal FastLAS 
task $T' = \langle B, M, E \rangle$
by performing the following transformation:
  
For each example 
$e = \langle \eid, \langle \epiinc, \epiexc \rangle, \eraw \rangle \in E^*$,
let $z_e$ be the corresponding ground truth latent concepts 
for the elements of $\eraw$, then we can 
construct the WCDPI $e = \langle \eid, \infty, \langle \epiinc, \epiexc \rangle,
z_{e^*} \rangle$
and add this to the set $E$ in $T'$.

Intuitively, $T'$ represent the normal 
FastLAS learning task 
that uses the ground truth latent concepts of the raw 
data. 
\end{definition}

Having defined a transformation of a NeuralFastLAS task $T$ to a fully symbolic 
task $T'$, we can now define the notion of symbolic correctness of a NeuralFastLAS 
solution:

\begin{definition}
We say that a solution $H^*$ to a NeuralFastLAS task $T$ is correct if $H^*$ is also an optimal solution to the collapse of $T$, $T'$.
\end{definition}

Note that this is different to the notion of an optimal solution, which 
aims to maximize the scoring function.

In order to maintain correctness guarantees across the stages,
we are able to prove that:

\begin{theorem}
  \label{theorem:g_containment}
  If $T'$ be the collapse of $T$, then $G(T') \subseteq G(T)$.
\end{theorem}
